A Critical Investigation of Deep Reinforcement Learning for Navigation

The navigation problem is classically approached in two steps: an exploration step, where map-information about the environment is gathered; and an exploitation step, where this information is used to navigate efficiently. Deep reinforcement learning (DRL) algorithms, alternatively, approach the problem of navigation in an end-to-end fashion. Inspired by the classical approach, we ask whether DRL algorithms are able to inherently explore, gather and exploit map-information over the course of navigation. We build upon Mirowski et al. [2017] work and introduce a systematic suite of experiments that vary three parameters: the agent's starting location, the agent's target location, and the maze structure. We choose evaluation metrics that explicitly measure the algorithm's ability to gather and exploit map-information. Our experiments show that when trained and tested on the same maps, the algorithm successfully gathers and exploits map-information. However, when trained and tested on different sets of maps, the algorithm fails to transfer the ability to gather and exploit map-information to unseen maps. Furthermore, we find that when the goal location is randomized and the map is kept static, the algorithm is able to gather and exploit map-information but the exploitation is far from optimal. We open-source our experimental suite in the hopes that it serves as a framework for the comparison of future algorithms and leads to the discovery of robust alternatives to classical navigation methods.

==> background.tex <==
Our problem formulation is based on the work of \citet{MiPaViICLR2017}. 
For completeness, we summarize the technical setup here.
For additional details regarding the setup, we refer the reader to \citet{MnBaMiICML2016,MiPaViICLR2017}.

The problem of navigation is formulated as an interaction between an environment and an agent.
At time $t$ the agent takes an action $\actt \in \Action$ and observes observation $\obst \in \Obs$ along with a reward $\rewt \in \R$.
We assume the environment to be a Partially Observable Markov Decision Process (POMDP).
In a POMDP, the future state of the environment, $\statetn \in \State$, is conditionally independent of all the past states, $\statehist$, given the current state $\statet$. It is further assumed that
$\obst$ and $\rewt$ are independent of previous states given current state $\statet$ and last action $\acttp$.
Formally, a POMDP is defined as a six tuple $(\Obs, \ObsFunc, \State, \Action, \Trans, \Rew)$ that is composed of an observation space $\Obs$, an observation function $\ObsFuncFull$, a state space $\State$, an action space $\Action$, a transition function $\TransFull$ and a reward function $\RewFull$.
For our problem setup, the observation space $\Obs$ is the space of an encoded feature vector that is generated from input image along with previous action and reward.
Action space $\Action$ contains four actions: rotate left, rotate right, move forward and move backward and reward function $\Rew$ is defined for each experiment so that reaching the goal location leads to high reward with auxiliary rewards to encourage certain kinds of behavior.

For DRL algorithms, the state space $\State$ is not hand tuned, but it is modeled as a vector of floats.
Additionally, instead of modeling observation function $\ObsFuncFull$ and $\TransFull$, a combined transition function $\TransObsFull$ is modeled to estimate the next state $\statetn$ and directly take previous observation and reward into account.
For policy-based DRL a policy function $\piDef$ and a value function $\ValueDef$ are also modeled.
All three functions $\TransObs$, $\pit$ and $\Valuet$ share most of the parameters such that $\theta_T \subseteq \theta_{\pi} \cap \theta_\Value$

The DRL objective is to estimate unknown weights $\theta = \theta_T \cup \theta_\pi \cup \theta_V$ that maximizes the expected future reward $\Ret_t = \sum_{k=t}^{t_{end} - t} \gamma^{k-t} r_k$ (where $\gamma$ is the discount factor) and is expressed as
%
\begin{align}
\theta^* = \arg\max_{\theta} \E[R_t] \,,
\end{align}
where $\E[.]$ denotes the expected value.
%
\input{fig-nav-a3c-horiz-figure}

\paragraph{Asynchronous Advantage Actor-Critic}
\def\charelig{\nabla_{\theta_\pi}\ln \pit(\acttn; \theta_\pi)}
In this work, we use the policy-based method called Asynchronous Advantage Actor-Critic (A3C) \citep{MnBaMiICML2016}, which allows weight updates to happen asynchronously in a multi-threaded environment.
It works by keeping a ``shared and slowly changing copy of target network'' that is updated every few iterations by accumulated gradients in each of the threads.
The gradients are never applied to the local copy of the weights; instead, a local copy of weights is periodically synced from the shared copy of target weights.
The gradient for the weight update is proportional to the product of \emph{advantage}, $R_t - \Value_t(\theta_\Value)$, and \emph{characteristic eligibility}, $\charelig$ \citep{WiML1992}, which update the weights as
\begin{align}
  \theta_\pi &\leftarrow \theta_\pi
  + \sum_{t \in \text{episode}}\alpha_\pi \nabla_{\theta_\pi}\ln \pit (R_t - \Value_t(\theta_\Value))
  \\
  \theta_\Value &\leftarrow \theta_\Value
  + \sum_{t \in \text{episode}} \alpha_\Value \frac{\partial (R_t - \Value_t(\theta_\Value))^2}
                  {\partial\theta_\Value}
                  \, .
\end{align}

For additional details of the A3C algorithm, we refer the reader to \citet{MnBaMiICML2016}.
%\input{fig-nav-a3c-vert-figure}
\paragraph{\NavAiiiCDiDiiL{}}
In this work, we use the \NavAiiiCDiDiiL{} architecture as proposed by \citet{MiPaViICLR2017}, which builds modifying the network architecture to have two LSTMs and with auxiliary outputs of depth predictions along with loop-closure predictions.
The schematic of the architecture is shown in Fig~\ref{fig:architectures}.
The architecture has three inputs: the current image $I_t$, previous action $\acttp$ and previous reward $\rewtp$.
As shown by \citet{MiPaViICLR2017}, the architecture improves upon vanilla A3C architecture by optimizing predictions for the auxiliary outputs of loop closure signal $L$ and predicted depth $D_1$ and $D_2$.
Since we use a smaller action space than \citet{MiPaViICLR2017} and our agent moves with constant velocity, we do not use velocity at the previous time step as an input signal.



==> fig-cnn-enc.tex <==
\begin{tikzpicture}
%\draw [use as bounding box] (0,0) rectangle (1.8in, 3in);
\node[] at (2.3, 2) (It) {$I_t$: 84x84x3};
\node[networknode, above=1.2 of It, text width=45, align=center] (c1) {conv\\
  3x3/2x2,32};
\node[above=1.2 of c1] (ft) {$o_t$: 256};
\draw [-stealth] (c1) edge [out=30, in=-30,looseness=2] node [right] {4x}(c1);
\draw [-stealth] (It) -- (c1);
\draw [-stealth] (c1) -- (ft);
\end{tikzpicture}


==> fig-fc-enc.tex <==
\begin{tikzpicture}
%\draw [use as bounding box] (0,0) rectangle (1.8in, 3in);
\node[] at (2.3, 2) (It) {$I_t$: 84x84x3};
\node[networknode, above=1.2 of It] (fc) {FC(256)};
\node[above=1.2 of fc] (ft) {$o_t$: 256};
\draw [-stealth] (It) -- (fc);
\draw [-stealth] (fc) -- (ft);
\end{tikzpicture}


==> fig-nav-a3c-vert-figure.tex <==
\begin{wrapfigure}[15]{r}{0.4\columnwidth}
\centering%
\scalebox{0.7}{\input{fig-nav-a3c-vert}}%
\caption{Modified \NavAiiiCDiDiiL{} (\cite{MiPaViICLR2017}) architecture.
Since we use a smaller action space than \cite{MiPaViICLR2017} and our agent moves with constant velocity, we do not use velocity at previous time step as input signal.}
\label{fig:architectures}
\end{wrapfigure}


==> fig-nav-a3c-vert.tex <==
\usetikzlibrary{positioning}
\begin{tikzpicture}
\node[networknode,fill=green!20] at (1.5, 3.5) (lstm2) {LSTM:64};
\node[networknode,fill=green!20,below=0.4 of lstm2] (lstm) {LSTM:256};
\node[networknode,fill=orange!20,below=0.4 of lstm]  (enc2) {\parbox{08ex}{CNN:32\\4x4/2x2}};
\node[networknode,fill=orange!20,below=0.4 of enc2]  (enc) {\parbox{08ex}{CNN:16\\8x8/4x4}};
\node[below=0.4 of enc, inputvar] (It) {$I_t$:84x84x3};
\node[left=0.1 of It,inputvar] (at) {$\acttp$};
\node[right=0.1 of It,inputvar]  (rt) {$\rewtp$};
\node [above=0.4 of lstm2,outvar] (V)  {$V$, $\pi$};
\node [shift={(-0,0)},left=0.3 of V,auxvar] (pi)  {$L$};
\node [shift={(-0,0)},right=0.3 of V,auxvar] (D)  {$D_2$};
\draw [-stealth] (It) edge (enc);
\draw [-stealth] (at) edge [in=-180,out=90,looseness=0.5] (lstm2);
\draw [-stealth] (enc2) edge [bend left=70,in=90,looseness=0.9] (lstm2);
\draw [-stealth] (enc) edge (enc2);
\draw [-stealth] (enc2) edge node [shift={(0,0.0)},left]{$o_t$} (lstm);
\draw [-stealth] (rt) edge  [bend right,in=-110,looseness=0.5] (lstm);
\draw [-stealth] (lstm) edge node[right=0.4,auxvar] (D1) {$D_1$} (lstm2);
\draw [-stealth] (lstm) edge [bend left] (D1);
\draw [-stealth] (lstm2) edge [bend right] (pi);
\draw [-stealth] (lstm2) edge  (V);
\draw [-stealth] (lstm2) edge [bend left] (D);
%\draw [use as bounding box] (0,-1.0) rectangle (3.0, 5.0);
\end{tikzpicture}

